Speeding up 6-DoF Grasp Sampling with Quality-Diversity

Recent advances in AI have led to significant results in robotic learning, including natural language-conditioned planning and efficient optimization of controllers using generative models. However, the interaction data remains the bottleneck for generalization. Getting data for grasping is a critical challenge, as this skill is required to complete many manipulation tasks. Quality-Diversity (QD) algorithms optimize a set of solutions to get diverse, high-performing solutions to a given problem. This paper investigates how QD can be combined with priors to speed up the generation of diverse grasps poses in simulation compared to standard 6-DoF grasp sampling schemes. Experiments conducted on 4 grippers with 2-to-5 fingers on standard objects show that QD outperforms commonly used methods by a large margin. Further experiments show that QD optimization automatically finds some efficient priors that are usually hard coded. The deployment of generated grasps on a 2-finger gripper and an Allegro hand shows that the diversity produced maintains sim-to-real transferability. We believe these results to be a significant step toward the generation of large datasets that can lead to robust and generalizing robotic grasping policies.

==> tex_files/figures/antipodal.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.6\columnwidth]{assets/antipodalV3.pdf}
  \caption{\textbf{QD-based vs standard prior-based sampling scheme.}}
  \label{fig:exp1_results}
\end{figure}


==> tex_files/figures/approach.tex <==

\begin{figure}[t]
  \centering
  \includegraphics[width=0.6\columnwidth]{assets/approachV3.pdf}
  \caption{\textbf{Approach method.} \hl{\textbf{TODO}}}
  \label{fig:genometo6dof}
\end{figure}


==> tex_files/figures/genome_to_6dof_principle.tex <==


\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{assets/qdg_prio_details.drawio.pdf}
  \caption{\textbf{Genome shaping for 6-DoF grasp sampling.} \hl{\textbf{TODO}}}
  \label{fig:genometo6dof}
\end{figure}




==> tex_files/figures/qd_priors_overall_principle.tex <==
% REPRENDRE ICI: en condensé dans le caption, et garder la description pour le results/discussion
\begin{figure*}[thpb]
  \centering
  \includegraphics[scale=1.0]{assets/schema_qdg6d_vue_ensemble_3.drawio.pdf}
  \caption{\textbf{Overall principle.} ...}
  \label{fig:qd_priors_overall_principle}
\end{figure*}






%\textbf{(a) wrong modelization of contacts} – the simulated scene consider a unique set of friction coefficient for each objects, while their surface are usually composed of different textures \textbf{(b) object's distribution of mass} – a wrong inertial matrix can result into impractical grasps ; \textbf{(c) errors in simulated models} – the mug handle can be grasped by tightening it within fingers, while this cannot be done on the real gripper; \textbf{(d) fragile grasps} – the exploratory power of QD methods sometimes result into grasps which are not robust enough to resist imprecisions inherent to real executions.











% determining the object's inertial matrix is not a trivial problem []. A wrong approximation of it might lead to unrealistic behaviors. A safe choice is to set the inertial matrix to $\mathbb{I}^3$, that is, to consider the whole mass is concentrated in the center of mass. This might however lead to non-transferable grasps: Fig. [].b shows an example in which the hand is balancing the bowl by touching it with the wrist, and catch the opposite side of the bowl in the air. This is obviously not verified in the real world, where similarly touching the bowl does not make it lift.

==> tex_files/figures/robotic_priors_principle.tex <==


\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\columnwidth]{assets/schema_qdg6d_a_priori.drawio.pdf}
  \caption{\textbf{Priors used in standard 6-DoF grasp sampling schemes.} \hl{\textbf{TODO:} 3 parties: contacts, approche, et antipodale}}
  \label{fig:robotic_priors_principle}
\end{figure}


